Rare Event Probability Learning by Normalizing Flows

A rare event is defined by a low probability of occurrence. Accurate estimation of such small probabilities is of utmost importance across diverse domains. Conventional Monte Carlo methods are inefficient, demanding an exorbitant number of samples to achieve reliable estimates. Inspired by the exact sampling capabilities of normalizing flows, we revisit this challenge and propose normalizing flow assisted importance sampling, termed NOFIS. NOFIS first learns a sequence of proposal distributions associated with predefined nested subset events by minimizing KL divergence losses. Next, it estimates the rare event probability by utilizing importance sampling in conjunction with the last proposal. The efficacy of our NOFIS method is substantiated through comprehensive qualitative visualizations, affirming the optimality of the learned proposal distribution, as well as a series of quantitative experiments encompassing $10$ distinct test cases, which highlight NOFIS's superiority over baseline approaches.

==> dummy.tex <==
\begin{algorithm}
  \caption{NOFIS}
  \label{alg:nofis}
  \begin{algorithmic}[1]
    \REQUIRE A data generating distribution $p\in\mathcal{P}^D$ and an integral region $\Omega=\{\mathbf{x}\in\mathbb{R}^D|g(\mathbf{x})\leq 0\}$.
    \ENSURE An estimation of the rare event probability $P_r=P[\Omega]$ defined in Eq.~(\ref{eq:question}).
    \STATE Define a NF characterized by a base distribution $q_0=p$, and a series of invertible transformations \text{\small $\{\mathbf{f}_i(\cdot)=\mathbf{f}(\cdot;\boldsymbol{\theta}_i):\mathbb{R}^D\to\mathbb{R}^D\}_{i=1}^{MK}$}.
    \STATE Choose hyper-parameters: (i) a strictly decreasing sequence $\{a_m\}_{m=1}^M$ satisfying $a_M=0$, and (ii) the temperature hyper-parameter $\tau>0$.
    \FOR{$m = 1$ to $M$}
      \STATE If $m\geq 2$, fix  \text{\small $\{\boldsymbol{\theta}_i\}_{i=1}^{(m-1)K}$} so that \text{\small $\{\mathbf{f}_i\}_{i=1}^{(m-1)K}$} are frozen.
      \FOR{$e=1$ to $E$} 
      \STATE Draw $N$ samples $\{\mathbf{z}_0^n\}_{n=1}^N$ from the NF base distribution $q_0=p$.
      \STATE Calculate the loss $D[q_{mK}||p^\tau_{m}]$ according to Eq.~(\ref{eq:kl_general}).
      \STATE Perform backward propagation and update the model parameters \text{\small $\{\boldsymbol{\theta}_{(m-1)K+i}\}_{i=1}^K$}.
      \ENDFOR
      % \STATE Train \text{\small $\{\mathbf{f}_{(m-1)K+i}\}_{i=1}^K$} according to Eq.~(\ref{eq:kl_general}), so that the random variable $\mathbf{z}_{mK}$ on the normalizing flow has a distribution $q_{mK}$ matched to $p_m^\tau$ shown in Eq. (\ref{eq:target_distribution_general}).
    \ENDFOR
    \STATE Draw $N_\text{IS}$ samples from $q_{MK}$ and calculate an IS estimator $P_r^{\text{IS}}$ based on Eq.~(\ref{eq:is}).
    \RETURN $P_r^{\text{IS}}$ as the estimation to $P_r$.
  \end{algorithmic}
\end{algorithm}

% Furthermore, our ablation study demonstrates that including an excessively long sequence \text\small{$\{a_m\}_{m=1}^M$} with a large value of $M$ does not significantly improve estimation accuracy but leads to an increased number of function calls.
 
